Data-Efficient Characterization of the Global Dynamics of Robot Controllers with Confidence Guarantees

This paper proposes an integration of surrogate modeling and topology to significantly reduce the amount of data required to describe the underlying global dynamics of robot controllers, including closed-box ones. A Gaussian Process (GP), trained with randomized short trajectories over the state-space, acts as a surrogate model for the underlying dynamical system. Then, a combinatorial representation is built and used to describe the dynamics in the form of a directed acyclic graph, known as {\it Morse graph}. The Morse graph is able to describe the system's attractors and their corresponding regions of attraction (\roa). Furthermore, a pointwise confidence level of the global dynamics estimation over the entire state space is provided. In contrast to alternatives, the framework does not require estimation of Lyapunov functions, alleviating the need for high prediction accuracy of the GP. The framework is suitable for data-driven controllers that do not expose an analytical model as long as Lipschitz-continuity is satisfied. The method is compared against established analytical and recent machine learning alternatives for estimating \roa s, outperforming them in data efficiency without sacrificing accuracy. Link to code: https://go.rutgers.edu/49hy35en

==> 07_supplementary_material.tex <==
\section{Supplementary Material}

More details about the systems and controllers are describe in this section. 
The state and control space limits are given in Table~\ref{table:systems}. 

\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{System} & \textbf{$X$} & $\mathbb{U}$ & \textbf{Bounds on $X$}  & \textbf{Bounds on $\mathbb{U}$} & \textbf{Controllers}\\ \hline
{\scriptsize\texttt{1D-Quadrotor}\cite{yuan2021safe} } & ${\scriptstyle(z, \dot{z})}$ & $T$ &$ {\scriptstyle[\{-10,-1\},\{10,1\}]}$ & ${\scriptstyle[-50,50]}$  & {\scriptsize\texttt{Learned} }\\ \hline
{\scriptsize\texttt{Pendulum} } & ${\scriptstyle(\theta, \dot{\theta})}$ & $\tau$ &$ {\scriptstyle[\{\pi,2\pi\},\{\pi,2\pi\}]}$ & ${\scriptstyle[0.6372,0.6372]}$ & {\scriptsize\texttt{Learned, LQR} }  \\ \hline
{\scriptsize\texttt{Mountain-Car} } & ${\scriptstyle(x, \dot{x})}$ & $\tau$ &$ {\scriptstyle[\{-1.2,-1.5\},\{0.6,1.5\}]}$ & ${\scriptstyle[-0.4, 0.4]}$ & {\scriptsize\texttt{Learned} }  \\ \hline
% \texttt{Ackermann} & $[-10,10] \cup [-10,10] \cup [-\pi,\pi]$  & $[-1.05,1.05] \cup [0,30]$ & \texttt{Learned, LQR, Corke} & $[0,0,\pi/2]$ \\ \hline
{\scriptsize\texttt{Ackermann \cite{corke2011robotics}} }& ${\scriptstyle(x,y,\theta)}$ & ${\scriptstyle(\gamma, V )}$ & ${\scriptstyle[\{-10,-10,-\pi\},\{10,10,\pi\}]}$  & ${\scriptstyle[\{-\frac{\pi}{3},0\},\{\frac{\pi}{3},30\}]}$ & \makecell{{{\scriptsize\tt Learned, LQR}}, \\{{\scriptsize\tt Corke}}} \\ \hline
{\scriptsize\texttt{Lunar-Lander} } & ${\scriptstyle(h, \dot{h}, m)}$ & $\dot{m}$ &$ {\scriptstyle[\{-1,-10,2134\},\{10,10,10334\}]}$ & ${\scriptstyle[0,9.765625]}$ & {\scriptsize\texttt{TOC} }  \\ \hline
{\scriptsize\texttt{Acrobot \cite{spong_acrobot}} }  & ${\scriptstyle(\theta_1, \theta_2, \dot{\theta_1}, \dot{\theta_2})}$ & $\tau_2$ & ${\scriptstyle[\{0,-\pi,-6,-6\},\{2\pi,\pi,6,6\}]}$ & ${\scriptstyle[14,14]}$ & {\scriptsize\texttt{Hybrid, LQR}}  \\ \hline
\end{tabular}


\caption{Systems and controllers considered in the evaluation.}
\label{table:systems}
% \vspace{-.45in}
\end{table}

\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{System} & \textbf{$X$} & \textbf{Controllers} & \textbf{Goal} \\ \hline
{\scriptsize\texttt{1D-Quadrotor}\cite{yuan2021safe} } & ${\scriptstyle(z, \dot{z})}$  & {\scriptsize\texttt{Learned} }& ${\scriptstyle[0,0]}$  \\ \hline
{\scriptsize\texttt{Pendulum} } & ${\scriptstyle(\theta, \dot{\theta})}$ &  {\scriptsize\texttt{Learned, LQR} }& ${\scriptstyle[0,0]}$  \\ \hline
{\scriptsize\texttt{Mountain-Car} } & ${\scriptstyle(x, \dot{x})}$ &  {\scriptsize\texttt{Learned} }& ${\scriptstyle[0.6,0]}$  \\ \hline
% \texttt{Ackermann} & $[-10,10] \cup [-10,10] \cup [-\pi,\pi]$  & $[-1.05,1.05] \cup [0,30]$ & \texttt{Learned, LQR, Corke} & $[0,0,\pi/2]$ \\ \hline
{\scriptsize\texttt{Ackermann \cite{corke2011robotics}} }& ${\scriptstyle(x,y,\theta)}$ & \makecell{{{\scriptsize\tt Learned, LQR}}, \\{{\scriptsize\tt Corke}}} & ${\scriptstyle[0,0,\frac{\pi}{2}]}$ \\ \hline
{\scriptsize\texttt{Lunar-Lander} } & ${\scriptstyle(h, \dot{h}, m)}$  & {\scriptsize\texttt{TOC} }& ${\scriptstyle[0,0,m_f]; m_f>2134}$  \\ \hline
{\scriptsize\texttt{Acrobot \cite{spong_acrobot}} }  & ${\scriptstyle(\theta_1, \theta_2, \dot{\theta_1}, \dot{\theta_2})}$ & {\scriptsize\texttt{Hybrid, LQR}} & ${\scriptstyle[0,\pi,0,0]}$  \\ \hline
\end{tabular}


\caption{Systems and controllers considered in the evaluation.}
\label{table:systems}
% \vspace{-.45in}
\end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \textbf{System} & \textbf{$X$} & $\mathbb{U}$ & \textbf{Bounds on $X$}  & \textbf{Bounds on $\mathbb{U}$} & \textbf{Controllers} & \textbf{Goal} \\ \hline
% {\scriptsize\texttt{1D-Quadrotor}\cite{yuan2021safe} } & ${\scriptstyle(z, \dot{z})}$ & $T$ &$ {\scriptstyle[\{-10,-1\},\{10,1\}]}$ & ${\scriptstyle[-50,50]}$  & {\scriptsize\texttt{Learned} }& ${\scriptstyle[0,0]}$  \\ \hline
% {\scriptsize\texttt{Pendulum} } & ${\scriptstyle(\theta, \dot{\theta})}$ & $\tau$ &$ {\scriptstyle[\{\pi,2\pi\},\{\pi,2\pi\}]}$ & ${\scriptstyle[0.6372,0.6372]}$ & {\scriptsize\texttt{Learned, LQR} }& ${\scriptstyle[0,0]}$  \\ \hline
% {\scriptsize\texttt{Mountain-Car} } & ${\scriptstyle(x, \dot{x})}$ & $\tau$ &$ {\scriptstyle[\{-1.2,-1.5\},\{0.6,1.5\}]}$ & ${\scriptstyle[-0.4, 0.4]}$ & {\scriptsize\texttt{Learned} }& ${\scriptstyle[0.6,0]}$  \\ \hline
% % \texttt{Ackermann} & $[-10,10] \cup [-10,10] \cup [-\pi,\pi]$  & $[-1.05,1.05] \cup [0,30]$ & \texttt{Learned, LQR, Corke} & $[0,0,\pi/2]$ \\ \hline
% {\scriptsize\texttt{Ackermann \cite{corke2011robotics}} }& ${\scriptstyle(x,y,\theta)}$ & ${\scriptstyle(\gamma, V )}$ & ${\scriptstyle[\{-10,-10,-\pi\},\{10,10,\pi\}]}$  & ${\scriptstyle[\{-\frac{\pi}{3},0\},\{\frac{\pi}{3},30\}]}$ & \makecell{{{\scriptsize\tt Learned, LQR}}, \\{{\scriptsize\tt Corke}}} & ${\scriptstyle[0,0,\frac{\pi}{2}]}$ \\ \hline
% {\scriptsize\texttt{Lunar-Lander} } & ${\scriptstyle(h, \dot{h}, m)}$ & $\dot{m}$ &$ {\scriptstyle[\{-1,-10,2134\},\{10,10,10334\}]}$ & ${\scriptstyle[0,9.765625]}$ & {\scriptsize\texttt{TOC} }& ${\scriptstyle[0,0,m_f]; m_f>2134}$  \\ \hline
% {\scriptsize\texttt{Acrobot \cite{spong_acrobot}} }  & ${\scriptstyle(\theta_1, \theta_2, \dot{\theta_1}, \dot{\theta_2})}$ & $\tau_2$ & ${\scriptstyle[\{0,-\pi,-6,-6\},\{2\pi,\pi,6,6\}]}$ & ${\scriptstyle[14,14]}$ & {\scriptsize\texttt{Hybrid, LQR}} & ${\scriptstyle[0,\pi,0,0]}$  \\ \hline
% \end{tabular}


% \caption{\small Systems and controllers considered in the evaluation.}
% \label{table:systems}
% % \vspace{-.45in}
% \end{table}

% add the description of “Hybrid controller”, L-LQR, L-SOS, in the supplemental material?
\textbf{Hybrid controller}
Given two controllers $u_1(x), u_2(x), x\in X$, a hybrid controller applies one controller in predetermined subsets of the state space $X_1,X_2 \subset X$, i.e.: $\dot{x}_{t+1} =\begin{cases} f(x_t,u_1) & x_t \in {X}_1 \\f(x_t,u_2) & x_t \in {X}_2\end{cases}$.
% A Hybrid controller for the Acrobot uses the Learned controller to drive the system to a relaxed goal distance, from where LQR takes ove

\textbf{Alternative methods}
Two lypunov-based analytical methods --\texttt{L-LQR} and \texttt{L-SoS}-- are used as comparison (as done in \cite{farsi2022piecewise,richards2018lyapunov}). Both methods use a linearized, unconstrained form of the dynamics to obtain a Lyapunov function (LF). \texttt{L-LQR} uses the solution of the Lyapunov equation $v_{LQR}(x)=x^TPx$ while \texttt{L-SoS} computes the LF according to $v_{sos}(x)=m(x)^TQm(x)$ where $m(x)$ are monomials on $x$ and $Q$ is a positive semidefinite matrix. The SoS problem is solved using SOSTOOLS \cite{prajna2002introducing} with SeDuMi \cite{sturm1999using} as the SDP solver. These methods cannot be used with data-driven controllers (like {\tt Learned}) since they require a closed-form expression for the controller. 
 
 \begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{figs/Lander_top_RoA.png}
    \includegraphics[width=\columnwidth]{figs/Lander_time10_14_box_ptwise_-10_300_RoA.png}
    \includegraphics[width=\columnwidth]{figs/Lander_time10_14_box_ptwise_-10_300_class_RoA.png}
    \caption{RoAs for the Lander found by: (left) {\tt Top-MG}; (middle) {\tt GP-MG} with Matérn kernel; and (right) {\tt GP-MG} with logistic regression together with Matérn kernel.}
    \label{fig:Lander}
\end{figure}



\begin{figure}%{l}{0.6\textwidth}
    \centering
    % \vspace{-0.15in}
    \includegraphics[width=\columnwidth]{figs/mountain_car_lc_time5_10.pdf}
    \includegraphics[width=\columnwidth]{figs/Car_moun_5.png}
    % \includegraphics[width=0.15\textwidth]{figs/mountain_car_lc_time10_10.pdf}
    \includegraphics[width=\columnwidth]{figs/Car_moun_10.png}
    \caption{Morse graph and RoA for the Car over terrain system: (left) Morse graph for short trajectories with time duration $0.5$ seconds and (middle) RoAs; (right) RoA for short trajectories with time duration $1$ seconds and Morse graph with only one node that represents the attractor.}
    \label{fig:Car_Top}
    % \vspace{-0.15in}
\end{figure}

==> Draft_of_Jacobian.tex <==

--------- Jacobian ---------

Two outer approximations are constructed based on the information GP provides. One leads to pointwise probability confidence (typical application of GP theory) and another presents overall probability confidence (bounds on probability given by GP derivatives). The former outer approximation is defined as follows.

Another possibility is defining an outer approximation with an associated probabilistic bound of the overall global dynamics. The key ingredient is the derivative of the trained GP, being also another Gaussian process, denote by $\eta$. A new multivalued map is constructed as follows.

Select a set $S$ such that $S\subset C(\cX)$ and $\mathrm{d}(S, C(\cX)\backslash S) = \mathrm{d_H}(S, C(\cX)\backslash S)=d$, where $\mathrm{d_H}$ is the Hausdorff distance. Hence $S$ is equally spaced. Now define 
\[B(v) =
\left\{\begin{array}{ll}
 \{x \in \mathbb{R}^N \ |\ \mathrm{d}(E^\delta_{\Sigma(\mu(v))},x)\leq dL(v)/2\}   & \text{ if } v\in S,\\
    E^\delta_{\Sigma(v)} & \text{ if } v\in C(\cX)\backslash S,
\end{array}\right.\]
where 
$L(v)=\mathrm{max}\{||\eta_z(\mu)|| \ |\ z\in C(\cX) \text{ and }  \mathrm{d}(v,z) \leq d/2 \}$ and $\eta_z(\mu)$ is the Jacobian of $\mu$ at $z$. 

Finally, the outer approximation is defined by 
\[
\cF_J(\xi) := \left\{ \xi' \mid  \xi' \cap B(v) \neq \emptyset\  \text{ for }\ v\in C(\xi)  \right\}, 
\] 
denote by {\it global confidence map}.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/F_J.pdf}
    \caption{Global confidence map $\cF_J$}
    \label{fig:F_J}
\end{figure}


% To provide a lower bound on the confidence of our characterization of dynamics, the Mat\'ern kernels with $\nu>2$ \cite{St99} are selected for this paper. Such kernels have the following bounds in its derivatives: 
% there exists constants $a,b>0$ such that for any $L>0$ we have
% \begin{equation}\label{eq:L}
% \mathbb{P}\left(\forall x\in X,\   \|\eta(x)\|\leq L\right)> \left( 1-ae^{-(\frac{L}{b})^2} \right)^{d^2}.
% \end{equation}
% (cf.\ \cite[Theorem 5]{GhRo06}). 


----- Experiments -----



%-------- Pendulum - LQR
\textbf{Pendulum LQR:}

The dynamical system of pendulum LQR setting: time 1, subdivision 12

\textbf{Multivalued Map F\_J:}

We randomly select 300 initial points and run Gaussian Process (Matern + Whitenoise) as the initial surrogate model. We use predicted maps for box enlarging with 1 standard deviation to get dynamics. In the adaptive adding points procedure, we select 10 points from (1) boundary parts (Vol value and region restriction) and (2) center attractor part in each step. Especially, jacobian matrix based on Gaussian process model is used to estimate Lipchizt constant K.

Figure \ref{fig:initial300} shows the transferred pendulum lqr data.

\begin{figure}[H]
  \centering
  \includegraphics[width=.6\linewidth]{figs/pendulum_lqr_jacobian/initial_300.png}
  \caption{Initial 300 Points}
\label{fig:initial300}
\end{figure}

Figure \ref{fig:initial_J} shows the standard deviation, error and Jacobian norm at Step 0.

\begin{figure}[H]
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step0_sd.png}
  \caption{Standard Deviation}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step0_error.png}
  \caption{Error}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step0_J.png}
  \caption{Jacobian}
\end{subfigure}%
\caption{Initial 300 points with 1*std}
\label{fig:initial_J}
\end{figure}

Figure \ref{fig:step0_J} shows the dynamic plot with 300 random sampling points.

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step0_dyn.png}
  \caption{Dynamics}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step0_morse.png}
  \caption{Morse Set}
\end{subfigure}
\caption{With 1*std}
\label{fig:step0_J}
\end{figure}

Figure \ref{fig:step1_30_J} shows the dynamic plot in step 15 and step 30.

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step15_dyn.png}
  \caption{Step 15}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step30_dyn.png}
  \caption{Step 30}
\end{subfigure}
\caption{With 1*std}
\label{fig:step1_30_J}
\end{figure}

Figure \ref{fig:step30_des_J} shows the standard deviation, error and Jacobian norm at Step 30.

\begin{figure}[H]
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step30_sd.png}
  \caption{Standard Deviation}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step30_error.png}
  \caption{Error}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step30_J.png}
  \caption{Jacobian}
\end{subfigure}%
\caption{Step 30}
\label{fig:step30_des_J}
\end{figure}

Figure \ref{fig:step30_J} shows the standard deviation after adding 300 points and the dynamic plot with 2*sd uncertainty.

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step30_dyn_1.png}
  \caption{Dynamics}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step30_morse_1.png}
  \caption{With 2*sd}
\end{subfigure}
\caption{After Step 30}
\label{fig:step30_J}
\end{figure}

Figure \ref{fig:step31_60_J} shows the dynamic plot in step 45 and step 60. 

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step45_dyn.png}
  \caption{Step 45}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step60_dyn.png}
  \caption{Step 60}
\end{subfigure}
\caption{With 2*std}
\label{fig:step31_60_J}
\end{figure}

Figure \ref{fig:step60_des_J} shows the standard deviation, error and Jacobian norm at Step 60.

\begin{figure}[H]
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step60_sd.png}
  \caption{Standard Deviation}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step60_error.png}
  \caption{Error}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step60_J.png}
  \caption{Jacobian}
\end{subfigure}%
\caption{Step 60}
\label{fig:step60_des_J}
\end{figure}

Figure \ref{fig:step60_J} shows dynamics and the morse graph after adding 600 points and the dynamic plot with 2*sd uncertainty.

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step60_dyn_revise.png}
  \caption{Dynamics}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step60_morse.png}
  \caption{Morse Set}
\end{subfigure}
\caption{After Step 60}
\label{fig:step60_J}
\end{figure}

The following table \ref{tab:vol_J} shows the morse set volume and roa volume.

\begin{table}[h]
    \centering
    \begin{tabular}{ | l | l | l |l | }
    \hline
     Morse Set & Set Vol & Tile Vol & Roa Vol \\
     \hline
     0  & 0.617  & 19.296 & 19.913 \\
     \rowcolor{yellow}
     1  & 0.154  & 28.298 & 28.452 \\
     2  & 0.829  & 4.087 & 4.916 \\
     3  & 1.388  & 19.065 & 20.452 \\
     4  & 0.81  & 4.395 & 5.205 \\
     5  & 0.019  & N/A &  0.019 \\
    \hline
    \end{tabular}
    \caption{Volume Summary}
    \label{tab:vol_J}
\end{table}

Figure \ref{fig:initial300_trans} shows the transferred pendulum lqr data.

\begin{figure}[H]
  \centering
  \includegraphics[width=.6\linewidth]{figs/pendulum_lqr_jacobian/initial300_trans.png}
  \caption{Transfered Initial 300 Points}
\label{fig:initial300_trans}
\end{figure}

Figure \ref{fig:step60_trans_J} shows the dynamics and morse graph after adding 600 points and the dynamic plot with 2*sd uncertainty, based on non-periodic data.

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step60_dyn_trans.png}
  \caption{Dynamics}
\end{subfigure}%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_jacobian/step60_morse_trans.png}
  \caption{Morse Set}
\end{subfigure}
\caption{After Step 60}
\label{fig:step60_trans_J}
\end{figure}

The following table \ref{tab:vol_trans_J} shows the morse set volume and roa volume.
 
\begin{table}[h]
    \centering
    \begin{tabular}{ | l | l | l |l | }
    \hline
     Morse Set & Set Vol & Tile Vol & Roa Vol \\
     \hline
     -1 & N/A    & N/A  & 2.467\\
     0  & 2.255  & 18.448 & 20.703 \\
     
     1  & 0.289  & 27.488 & 27.777 \\
     2  & 1.022  & 3.585 & 4.607 \\
     3  & 0.617  & 19.585 & 20.202 \\
     4  & 0.733  & 2.349 & 3.082 \\
     5  & 0.019  & 0.039 &  0.058 \\
     6  & 0.019  & 0.039 &  0.058\\
    \hline
    \end{tabular}
    \caption{Volume Summary}
    \label{tab:vol_trans_J}
\end{table}

\textbf{Multivalued Map Box\_ptwise:}

Figure \ref{fig:initial_P} shows the dynamic plot with 300 random sampling points.

\begin{figure}[H]
\begin{subfigure}{.35\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step0_dyn.png}
  \caption{Dynamics}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step0_morse.png}
  \caption{Morse Set}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step0_sd.png}
  \caption{Standard Deviation}
\end{subfigure}%
\caption{Initial 300 points with 0.25*std}
\label{fig:initial_P}
\end{figure}

Figure \ref{fig:step1_30_P} shows the dynamic plot in step 15 and step 30.

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step15_dyn.png}
  \caption{Step 15}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step30_dyn.png}
  \caption{Step 30}
\end{subfigure}
\caption{With 0.25*std}
\label{fig:step1_30_P}
\end{figure}

Figure \ref{fig:step30_P} shows the standard deviation after adding 300 points and the dynamic plot with 1*sd uncertainty.

\begin{figure}[H]
\begin{subfigure}{.6\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step30_sd.png}
  \caption{Standard Deviation}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step30_dyn_0.png}
  \caption{With 1*sd}
\end{subfigure}
\caption{After Step 30}
\label{fig:step30_P}
\end{figure}

Figure \ref{fig:step31_60_P} shows the dynamic plot in step 45 and step 60. 

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step45_dyn.png}
  \caption{Step 45}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step60_dyn.png}
  \caption{Step 60}
\end{subfigure}
\caption{With 1*std}
\label{fig:step31_60_P}
\end{figure}

Figure \ref{fig:step60_P} shows the standard deviation after adding 600 points and the dynamic plot with 2*sd uncertainty.

\begin{figure}[H]
\begin{subfigure}{0.55\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step60_sd.png}
  \caption{Standard Deviation}
\end{subfigure}%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step60_dyn_1.png}
  \caption{With 2*sd}
\end{subfigure}
\caption{After Step 60}
\label{fig:step60_P}
\end{figure}

Figure \ref{fig:step61_90_P} shows the dynamic plot in step 75 and step 90. 

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step75_dyn.png}
  \caption{Step 75}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step90_dyn.png}
  \caption{Step 90}
\end{subfigure}
\caption{With 2*std}
\label{fig:step61_90_P}
\end{figure}

Figure \ref{fig:step90_P} shows the standard deviation after adding 900 points and the morse graph.

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step90_sd.png}
  \caption{Standard Deviation}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step90_morse.png}
  \caption{Morse Set}
\end{subfigure}
\caption{After Step 90}
\label{fig:step90_P}
\end{figure}

Similarly, we also apply non-periodic dynamical system data. Figure \ref{fig:step90_trans_P} shows the dynamics and morse graph after adding 1200 points and the dynamic plot with 2*sd uncertainty.

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step90_dyn_trans.png}
  \caption{Dynamics}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figs/pendulum_lqr_ptwise/step90_morse.png}
  \caption{Morse Set}
\end{subfigure}
\caption{After Step 90}
\label{fig:step90_trans_P}
\end{figure}

The following table \ref{tab:vol_trans_P} shows the morse set volume and roa volume.

\begin{table}[h]
    \centering
    \begin{tabular}{ | l | l | l |l | }
    \hline
     Morse Set & Set Vol & Tile Vol & Roa Vol \\
     \hline
     -1 & N/A & N/A & 2.31\\
     \rowcolor{yellow}
     0  & 1.21  & 26.97 & 28.18 \\
     1  & 8.23  & 15.84 & 24.07 \\
     2  & 5.9  & 18.48 & 24.38 \\
    \hline
    \end{tabular}
    \caption{Volume Summary}
    \label{tab:vol_trans_P}
\end{table}


\textbf{Ackermann -- Learned controller:}

The dynamical system of ackermann learned controller setting: time 1, subdivision 20.

\textbf{Multivalued Map Box\_ptwise:}

We randomly select 1000 initial points and run Gaussian Process as the initial surrogate model. Since predicted standard deviations based on the Gaussian process models are small, 2*std is used in multivalued map and we randomly sample another 1000 points as the second step to compare results.

With initial 1000 points and Gaussian process models, we are able to find one attractor. The morse set volume is 17, which is large because the output from ackermann learned controller would spread from $[0, 0, -\pi]$ to $[0, 0, \pi]$. The morse set of the attractor includes 7095 boxes around the target point $[0, 0, 0]$, especially along the third dimension from $-\pi$ to $\pi$.

After adding 1000 point and re-building Gaussian process models, we are also able to find one attractor. The morse set volume and the region of attractor volume are the same as initial ones.

If we set ackermann learnerd controller with time 40 to make the output focus around 0. With initial 1000 points, the morse set volume becomes 0.57, including 240 boxes around $[0, 0, 0]$.

\textbf{Multivalued Map F\_J:}

\textbf{Acrobot LQR:}

The dynamical system of acrobot LQR setting: time 14, subdivision 20.

\textbf{Multivalued Map Box\_ptwise:}

We randomly select 1000 initial points and run Gaussian Process as the initial surrogate model. At time 14, acrobot LQR dynamical system is able to move points to the target point $[\pi, 0, 0, 0]$, which makes it easier to build Gaussian process models. Since predicted standard deviations based on the Gaussian process models are small, 2*std is used in multivalued map and we randomly sample another 1000 points as the second step to compare results.

With initial 1000 points and Gaussian process models, we are able to find one attractor. The morse set volume is 0.0867 (include 16 boxes around the target point $[\pi, 0, 0, 0]$), while the region of attractor volume is 5684.89 (the volume of the whole space).

After adding 1000 point and re-building Gaussian process models, we are also able to find one attractor. The morse set volume and the region of attractor volume are the same as initial ones.

\textbf{Multivalued Map F\_J:}


\textbf{Lander:}



\textbf{Car over terrain:}






% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{\textwidth}
%          \includegraphics[width=.195\textwidth]{example-image-a}
%          \includegraphics[width=.195\textwidth]{example-image-a}
%          \includegraphics[width=.195\textwidth]{example-image-a}
%          \includegraphics[width=.195\textwidth]{example-image-a}
%          \includegraphics[width=.195\textwidth]{example-image-a}
%          \label{fig:systems}
%     \end{subfigure}\\
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \subsection{Qualitative case studies}



